Distributional Model Equivalence for Risk-Sensitive Reinforcement Learning

We consider the problem of learning models for risk-sensitive reinforcement learning. We theoretically demonstrate that proper value equivalence, a method of learning models which can be used to plan optimally in the risk-neutral setting, is not sufficient to plan optimally in the risk-sensitive setting. We leverage distributional reinforcement learning to introduce two new notions of model equivalence, one which is general and can be used to plan for any risk measure, but is intractable; and a practical variation which allows one to choose which risk measures they may plan optimally for. We demonstrate how our framework can be used to augment any model-free risk-sensitive algorithm, and provide both tabular and large-scale experiments to demonstrate its ability.

==> appendices/planning-algorithms-used.tex <==
\section{Planning algorithms used}\label{sec:PlanningAlgoUsed}

\begin{algorithm}
   \caption{Mean-variance value iteration}
\begin{algorithmic}
   \STATE {\bfseries Input:} Variance weight $\lambda$, error threshold $\theta$, MDP $(\stateSpace,\actionSpace,\transitionFn,\rewardFn,\gamma)$
   \STATE Initialize $V(x) = 0$ for all $x\in\stateSpace$.
   \STATE Initialize ${Var}(x) = 0$ for all $x\in\stateSpace$.
   \REPEAT
   \FOR{each $x\in \stateSpace$}
   \STATE $V_{tmp}(x,a) = \E_{R\sim \rewardFn(x,a)}\left[R\right]+\gamma \sum_{x'\in\stateSpace}\transitionFn(x'|x,a)\,V(x')$\vspace{3pt}
   \STATE $Var_{tmp}(x,a) = \E_{R\sim \rewardFn(x,a)}\left[R^2\right]+2\gamma \sum_{x'\in\stateSpace}\transitionFn(x'|x,a)\,V(x')+\gamma^2\sum_{x'\in\stateSpace}\transitionFn(x'|x,a)\,Var(x')$\vspace{3pt}
    \STATE $meanVar(x,a) = V_{tmp}(x,a)-\lambda Var_{tmp}(x,a)$\vspace{3pt}
    \STATE $\pi(x) = \arg\max_{a\in \actionSpace}meanVar(x,a)$\vspace{3pt}
    \STATE $V_{old}(s) = V(s)$\vspace{3pt}
    \STATE $Var_{old}(s) = Var(s)$\vspace{3pt}
    \STATE $V(s)=V_{tmp}(\pi(s))$\vspace{3pt}
    \STATE $Var(s)=Var_{tmp}(\pi(s))$\vspace{3pt}
    \STATE $\Delta =\max(\Delta, |Var(s)-Var_{old}(s)|, |V(s)-V_{old}(s)|)$
   \ENDFOR
   \UNTIL{$\Delta < \theta$}
   \STATE {\bf return} $\pi$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
   \caption{CVaR value iteration}
\begin{algorithmic}
   \STATE {\bfseries Input:} Level $\tau$, number of iterations $num_iters$, probability distribution representation $\F$, projection $\Pi_\F$, discretization width $\varepsilon$, MDP $(\stateSpace,\actionSpace,\transitionFn,\rewardFn,\gamma)$ with reward bound $R_{\text{max}}$, starting state $x_0$\vspace{4pt}
   \STATE Let $\B_\varepsilon$ be a discretization of $[-R_{\text{max}}/(1-\gamma),R_{\text{max}}/(1-\gamma)]$ into intervals of length $\varepsilon$
   \STATE Initialize $\eta(x,a,b) = \Pi_\F\delta_0$ for all $x\in\stateSpace$, $a\in\actionSpace$, $b\in \B_\varepsilon$
   \STATE $b=0$
   \STATE $k=0$
   \REPEAT
   \FOR{each $x\in \stateSpace$}
   % \STATE $G(x,a)=\E[\eta(x,a,b)]$
   \STATE $a'=\arg\min_{a\in\actionSpace}\left[\max(b-\frac1\tau \E_{Z\sim \eta(x,a,b)}[Z],0)\right]$
   \FOR{each $a\in \actionSpace$}
   \STATE $\eta(x,a,b)=\Pi_\F\left(\sum_{x'\in\stateSpace}\transitionFn(x'|x,a)\,\E_{R\sim \rewardFn(x,A)}\left[(b_{,\gamma})_{\#}\eta(x', a', b)\right]\right)$
   \vspace{3pt}
    \ENDFOR
    \STATE $V_{old}(s) = V(s)$\vspace{3pt}
    \STATE $Var_{old}(s) = Var(s)$\vspace{3pt}
    \STATE $V(s)=V_{tmp}(\pi(s))$\vspace{3pt}
    \STATE $Var(s)=Var_{tmp}(\pi(s))$\vspace{3pt}
    \STATE $\Delta =\max(\Delta, |Var(s)-Var_{old}(s)|, |V(s)-V_{old}(s)|)$
   \ENDFOR
   \UNTIL{$k = num_iters$}
   \STATE {\bf return} $\pi$
\end{algorithmic}
\end{algorithm}




==> sections/acknowledgements.tex <==
\section{Acknowledgements}

We would like to thank the members of the Adaptive Agents Lab who provided feedback on a draft of this paper. AMF acknowledges the funding from the Canada CIFAR AI Chairs program, as well as the support of the Natural Sciences and Engineering Research Council of Canada (NSERC) through the Discovery Grant program (2021-03701). MAE was supported by NSERC Grant [2019-06167], CIFAR AI Chairs program, and CIFAR AI Catalyst grant. Resources used in preparing this research were provided, in part, by the Province of Ontario, the Government of Canada through CIFAR, and companies sponsoring the Vector Institute.

